Compressed Online Dictionary Learning for Fast fMRI Decomposition

We present a method for fast resting-state fMRI spatial decomposi-tions of very large datasets, based on the reduction of the temporal dimension before applying dictionary learning on concatenated individual records from groups of subjects. Introducing a measure of correspondence between spatial decompositions of rest fMRI, we demonstrates that time-reduced dictionary learning produces result as reliable as non-reduced decompositions. We also show that this reduction significantly improves computational scalability.

==> matplotlibrc <==
backend: pgf

pgf.texsystem: pdflatex
text.usetex: True
font.family: serif
font.serif:
font.sans-serif:
font.monospace:

axes.labelsize: 9
font.size: 9
legend.fontsize: 7
xtick.labelsize: 7
ytick.labelsize: 7
figure.figsize: 3.38582676075, 2.0925560181624587
figure.dpi: 600

pgf.preamble: \usepackage[utf8x]{inputenc},\usepackage[T1]{fontenc}
# figure.autolayout: True

savefig.dpi: 600
savefig.pad_inches  : 0.

